Experimental study of aerosol deposition in distal lung bronchioles

The deposition of micron particles finds importance in meteorology and several engineering applications such as deposition of dust in gas lines, carbon deposition in engine exhaust, designing effective air-cleaning systems and estimating deposition of inhaled drug or atmospheric pollutants to determine its consequences on human health. Although the existing literature on deposition in straight tubes is quite mature, an experimental study on deposition in micro capillaries with a wide ranges of Re that models particle dynamics in lungs, is missing. The deposition of atmospheric pollutants and nebulized drugs in the lung depends on various biological factors such as flow properties, lung morphology, breathing patterns, particle properties, deposition mechanism, etc. To complicate matters, each breath manifests flows spanning a wide range of Reynolds numbers in various regions of the lung. In this study, the deposition of nebulized aerosol was experimentally investigated in phantom bronchioles of diameters relevant to the 7th to the 23rd branching generations and over the entire range of Re manifest during one breathing cycle. The aerosol fluid was loaded with boron doped carbon quantum dots as a fluorophore. An aerosol was generated of this mixture fluid using an ultrasonic nebulizer, producing droplets of 6.5$\mu$m as the mean diameter. The amount of aerosol deposited on the bronchiole walls was measured using a spectrofluorometer. Finally, a universal bronchiole scale deposition model is proposed which can form the building block for lung-scale aerosol deposition prediction.

==> lineno/README <==
README
                      lineno.sty  v3.07

     $Id: README,v 3.5 2001/07/31 02:57:33 stephan Exp $

The LaTeX package lineno.sty provides line numbers on paragraphs.
After TeX has broken a paragraph into lines there will be line numbers
attached to them, with the possibility to make references through the
LaTeX \ref, \pageref cross reference mechanism.

% Copyright 1995--1999 Stephan I. B"ottcher <stephan@nevis1.columbia.edu>
%
% This program can be redistributed and/or modified under the terms
% of the LaTeX Project Public License Distributed from CTAN
% archives in directory macros/latex/base/lppl.txt; either
% version 1 of the License, or any later version.


Todo:

   ???

Changes:

   2001-07-30 SiB: [hyperref] option obsolete.
   2001-01-17 SiB: LaTeX class option [twocolumn] support
   2001-01-04 SiB: LaTeX class option [fleqn] support
   2000-12-18 SiB: longtable compatibility
   2000-07-01 SiB: extra \newlabel items, [hyperref] option
   2000-03-10 SiB: indirect call of \output, to work with multicol.
   1999-08-28 SiB: fixed the footnote problem using \holdinginserts
   1999-06-11 SiB: included the extensions into lineno.sty
   1999-03-02 SIB: Added LPPL License


Files:

   README        This file.
   COPYING       The LPPL header.
   lineno.sty    The package itself, ready to use.
   lineno.tex    The source documentation.
   ulineno.tex   The pathetic attempt of a users manual.

     As of version v3.00, the extension packages for lineno have all been
     incorporated into lineno.sty itself.  Except for itemrule.sty,
     which was removed.

Home:

   http://www.nevis.columbia.edu/~stephan/tex
   CTAN:macros/latex/contrib/supported/lineno


Author:

   Stephan I. B"ottcher <Stephan.Boettcher@desy.de>

Compatibility with other packages:

   wrapfig.sty   works since v2.05

   multicol.sty  works partly since 3.02.  
                 Do NOT use \linelabel.  Do NOT put a multicol in
                 internal vertical mode {table}, {figure}, etc.

   hyperref.sty  \ref to a \linelabel works since v3.03.

   longtable.sty broke with lineno.sty loaded, but not enabled.  
                 This is fixed in v3.04.

To print the documented source:

   Take the style-file `lineno.sty', and feed it to a Un*x shell.  (Or
   download the extracted source documentation `lineno.tex'.)

      csh> source ./lineno.sty
      sh>  . ./lineno.sty

   (Please ignore the error message at the beginning about the iffalse.)


Please have a look at a similar work of Michal Jaegermann and James
Fortune:
         CTAN:macros/latex/contrib/supported/numline/


